How Hackable Is Your Speech Quality Metric? A Corrected Protocol, a Benchmark, and What Patching Buys

Speech quality predictors are increasingly used as rewards, yet no agreed measure of their hackability exists. The usual measurement has two flaws. First, the perturbation reaches the predictor through a processing chain -- here a neural codec -- that shifts the score on its own, which scoring against the raw input charges to the attack. Referencing the unperturbed round trip instead changes measured hackability by up to a factor of four (0.31 to 0.08 for one defence). Second, one trained attacker is a sample, not a measurement: five attackers differing only in random seed reach success rates from 0.00 to 0.38 against one fixed predictor, so a defence claim needs the worst case over several. Under this protocol, four published predictors differ widely: NISQA is hacked on 90% of utterances, SSL-MOS on 21%, DNSMOS on 14% and UTMOS on 6%. We then audit a closed attack-detect-patch loop. It hardens the predictor only in its own attack space, by less than the spread between attackers; a random-perturbation baseline matches it; and it costs up to 0.30 system SRCC out of domain. Enhancers post-trained against patched predictors hack them far less (PESQ -0.03 versus -0.23). Code, preregistration and run outputs are released.

==> tables/table2.tex <==
% generated by analysis/paper_assets.py
\begin{tabular}{l c c c}
\toprule
& \multicolumn{2}{c}{BVCC test} & out-of-domain \\
\cmidrule(lr){2-3}
Predictor & sys SRCC & utt MSE & mean sys SRCC \\
\midrule
$R_0$ (no defense) & 0.922$\pm$0.004 & 0.234$\pm$0.011 & 0.731$\pm$0.006 \\
$R_1$ & 0.911$\pm$0.009 & 0.272$\pm$0.034 & 0.690$\pm$0.014 \\
$R_2$ & 0.918$\pm$0.003 & 0.272$\pm$0.006 & 0.682$\pm$0.008 \\
$R_3$ (EnCodec loop) & 0.920$\pm$0.001 & 0.272$\pm$0.022 & 0.637$\pm$0.046 \\
$R_3^{\mathrm{multi}}$ (multi-space) & 0.914$\pm$0.003 & 0.277$\pm$0.004 & 0.552$\pm$0.015 \\
noise pairs & 0.917$\pm$0.004 & 0.275$\pm$0.021 & 0.722$\pm$0.013 \\
PGD pairs & 0.909$\pm$0.001 & 0.274$\pm$0.023 & 0.635$\pm$0.009 \\
random-latent pairs & 0.922$\pm$0.004 & 0.298$\pm$0.049 & 0.696$\pm$0.010 \\
\bottomrule
\end{tabular}

